Stay Connected, Leave no Trace: Enhancing Security and Privacy in WiFi via Obfuscating Radiometric Fingerprints

The intrinsic hardware imperfection of WiFi chipsets manifests itself in the transmitted signal, leading to a unique radiometric fingerprint. This fingerprint can be used as an additional means of authentication to enhance security. In fact, recent works propose practical fingerprinting solutions that can be readily implemented in commercial-off-the-shelf devices. In this paper, we prove analytically and experimentally that these solutions are highly vulnerable to impersonation attacks. We also demonstrate that such a unique device-based signature can be abused to violate privacy by tracking the user device, and, as of today, users do not have any means to prevent such privacy attacks other than turning off the device. We propose RF-Veil, a radiometric fingerprinting solution that not only is robust against impersonation attacks but also protects user privacy by obfuscating the radiometric fingerprint of the transmitter for non-legitimate receivers. Specifically, we introduce a randomized pattern of phase errors to the transmitted signal such that only the intended receiver can extract the original fingerprint of the transmitter. In a series of experiments and analyses, we expose the vulnerability of adopting naive randomization to statistical attacks and introduce countermeasures. Finally, we show the efficacy of RF-Veil experimentally in protecting user privacy and enhancing security. More importantly, our proposed solution allows communicating with other devices, which do not employ RF-Veil.

==> figs/fig_evaluation.tex <==
% Figure 3-4



==> setup.tex <==
%\vspace{-4mm}
\subsection{SDR Implementation}
\label{s:setup}

%TODO the sender needs to use a sequence number
%TODO The receiver just checks if the incoming number is higher than the last one
%==> With this we can thwart replay attacks

\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{figs/setup.pdf}
	%\vspace{-2mm}	
	\caption{Schematic overview of the hardware setup.}
	\label{fig_setup}
	%        \vspace{-6mm}
\end{figure}

A simplified overview of the hardware used in our setup is depicted in Figure \ref{fig_setup}.
Each of the \gls{NI} USRPs (2954 R) is connected via PCI-E to a host machine running NI-Linux RT.
We use the 802.11 implementation by NI, which provides a PHY as well as a lower- and mid-MAC layer implementation\footnote{\blue{Link to AFW?}}. 
The NI 802.11 \gls{AFW} is separated into a host and an FPGA part, which communicate through FIFO data buffers. 
Figure \ref{fig_setup} also shows where the different layers of the protocols are implemented. 
Due to strict timing constraints, the MAC layer has been separated into lower MAC layer implemented on the FPGA while the middle and higher MAC layer are both implemented on the host. 

\textbf{Fingerprint Extraction. }
We chose to implement the fingerprint extraction solely on the host, as the CSI was already available through the \gls{T2H} FIFO \textit{Channel Estimation}.
The FIFO contains a 64 bit complex value for each of the measured 256 sub-carrier in a 80 MHz wide band. 
We implemented the fingerprinting algorithm proposed by Liu \textit{et al.} \cite{liu:2019} on a per-frame basis as a new module of the AFW. 


\textbf{Fingerprint Modification. } 
In order to modify the fingerprint we added a new FIFO, facilitating the exchange of an array of complex values from the host to the FPGA. 
We made use of the \gls{ICP} by NI to send packets containing the additional phase rotation to the FPGA. 
We then modified the TX-chain on the PHY in order to read the packets and to multiply each outgoing I/Q symbols with the corresponding phase rotation.


\textbf{Secure Fingerprinting Algorithm. }
We implemented the PoC of \Alg{} on top of the \textit{Fingerprint Extraction} and \textit{Fingerprint Modification} modules on the host. 
Once a packet is generated at the transmitter and passed down to the PHY, the MAC-address is used to obtain the corresponding information from the \gls{LUT} and to create the randomization sequence as well as the sequence number.
Those two elements are then multiplied and serve as input for the \textit{Fingerprint Modification} module, which takes care of pushing the values to the PHY.

On the receiver side, the CSI is written into the \textit{T2H Channel Estimation} FIFO at the PHY. 
The reception of the frame continues on the FPGA while the implementation of \Alg{} runs on the output of the FIFO on the host.
After the information for the random sequence generation is obtained and the randomization reverted, the fingerprint is calculated by \textit{Fingerprint Extraction} module.
The fingerprint is then passed to the \textit{Matcher}, which calculates the euclidean distance between the fingerprint of the frame and the known fingerprint for the MAC address. 
It is worth emphasizing here that implementing a more sophisticated matching-algorithm is possible but considered out of scope in this work.

%TODO is the last sentence here okay?

